Sequential Causal Imitation Learning with Unobserved Confounders

"Monkey see monkey do" is an age-old adage, referring to na\"ive imitation without a deep understanding of a system's underlying mechanics. Indeed, if a demonstrator has access to information unavailable to the imitator (monkey), such as a different set of sensors, then no matter how perfectly the imitator models its perceived environment (See), attempting to reproduce the demonstrator's behavior (Do) can lead to poor outcomes. Imitation learning in the presence of a mismatch between demonstrator and imitator has been studied in the literature under the rubric of causal imitation learning (Zhang et al., 2020), but existing solutions are limited to single-stage decision-making. This paper investigates the problem of causal imitation learning in sequential settings, where the imitator must make multiple decisions per episode. We develop a graphical criterion that is necessary and sufficient for determining the feasibility of causal imitation, providing conditions when an imitator can match a demonstrator's performance despite differing capabilities. Finally, we provide an efficient algorithm for determining imitability and corroborate our theory with simulations.

==> a_algorithm.tex <==

\begin{lemma}
    \label{lemma:fullvx}
    Suppose that there exists a sequential $\pi$-backdoor for $\bm{X}$. Then $\bm{X}\subseteq\textsc{FindOx}(\mathcal{G},\bm{X},Y)$.
\end{lemma}

\begin{proof}
    We first observe that keys can only be added to $\mathscr{O}^X$ in \Cref{alg:seq_pi_backdoor}. Furthermore, while the algorithm runs a loop in reverse temporal order, the outer "do" runs until there is no change in $\mathscr{O}^X$ for a pass through all of the variables.

    We can therefore do a proof by induction over $\bm{X}$ in reverse temporal order. In particular, on each successive pass of the outer loop, we focus on the element before it, $X_i\in \bm{X}$ and its ancestors - since adding elements to $\mathscr{O}^X$ can only help in the conditioning checks, the focus on reverse temporal order is, in a sense, a worst-case scenario of the algorithm being artificially limited.

    We will show that after the $i$th successive outer-loop, all elements of $X_{k-i+1},...,X_k$ will be in the set $keys(\mathscr{O}^X)$, as well as all elements that are not ancestors of $Y$ in $\mathcal{G}'_{k-i+1}$ of the ancestral graph of $Y$.

    In the first outer loop, we have $X_k\in \bm{X}$ that is last in temporal order. When performing the check for $X_k$, a conditioning check is performed ensuring that all values of the c-component of $\bm{X}$
    
    
    Suppose for contradiction that $V_j$ is not an ancestor of $Y$ in $\mathcal{G}'_{k-1}$ or is $X_k$, and yet $V_i\notin keys(\mathscr{O}^X)$. Since the check is performed in the ancestral graph of $Y$, the only way for this to be true is if all of its directed paths to $Y$ pass through $X_k$, and as such are cut when the parents of $X_k$ are replaced with the conditioning set $Z_k$. We therefore conclude that $V_i$ and has at least one directed path (possibly of size 0 if $V_i=X_k$) to $X_k$ in $\mathcal{G}$, and no element along any path from $V_i$ to $X_k$ is in $Z_k$ (otherwise it would be an ancestor of $Y$ in $\mathcal{G}'_{k-1}$). For $V_i$ to not be in $keys(\mathscr{O}^X)$, the algorithm's conditioning check must have failed somewhere along one of the directed paths to $X_k$. Call the node of failure $V_j$. The conditioning check ensures that all elements in the c-component of $V_j$ reachable without using colliders at elements in $\mathscr{O}^X$ are in $\before(X_i)$. Since the keys of $\mathscr{O}^X$ represent non-ancestors of $Y$, the check failing means that there is a path to an element of the c-component that is in $\before(X_k)$. Each collider that the path passes is either an ancestor of $Y$, and therefore either it, or one of its descendants must be in $\bm{Z}_k$, or was not yet added to $keys(\mathscr{O}^X)$, but it itself is not an ancestor of $Y$, in which case the same proof can be repeated using that element as $V_j$, since it would also fail the conditioning check. Since any conditioning set will have a path to an element before $X_k$, which itself is an ancestor of $Y$ in $\mathcal{G}'_{k-1}$, it and its descendants can't be part of a conditioning set $\bm{Z}_k$, meaning that there was a contradiction ($\bm{Z}_k$ was a d-separating set - since $X_k$ was the last element in temporal order, and we are in the ancestral graph of $Y$, it must satisfy condition (1).

    Now suppose we are on the $i$'th loop. After the first $i-1$ loops, all elements  $X_{k-i+1},...,X_k$ will be in the set $keys(\mathscr{O}^X)$, and all elements that are not ancestors of $Y$ in $\mathcal{G}'_{k-i}$ are also in $keys(\mathscr{O}^X)$.
    If $X_{k-i}$ satisfies condition (2) of the sequential $\pi$-backdoor, then it is already in $keys(\mathscr{O}^X)$, and any policy chosen will not have any effect on the elements that are ancestors of $Y$. 
    
    However, if it satisfies condition (1), we proceed in the same way as before (we show a shortened repeat here).
    Suppose for contradiction that $V_i$ is not an ancestor of $Y$ in $\mathcal{G}'_{k-i-1}$, but is not in $keys(\mathscr{O}^X)$ after the $i$th loop. Since all non-ancestors of $Y$ that don't have paths through $X_i$ were already in $keys(\mathscr{O}^X)$ after the $i-1$st loop, $V_i$ must have a directed path to $X_i$. For the algorithm to not include the element, the conditioning check must have failed at some node on one of the paths from $V_i$ to $X_i$. Call this element $V_j$. Once again, the conditioning $\bm{Z}_k$ that satisfies the sequential $\pi$-backdoor must block all elements of the c-component of $V_j$ that have directed paths to $Y$ which are reachable without conditioning on non-ancestors, which is violated if any such element comes before $X_i$. This is a contradiction, since the conditioning set satisfies the sequential $\pi$-backdoor. 
    
    We have therefore shown that after repeating the proof inductively for all variables, using $k$ passes of the algorithm through the nodes, we have $\bm{X}\subseteq\textsc{FindOx}(\mathcal{G},\bm{X},Y)$.
\end{proof}

The next theorem and proof will use the following definition of boundary nodes:
\boundarynodes*

\constructmfactor*

\begin{proof}
    We will perform a proof by induction over the algorithm's $\mathscr{O}^X$ map. Suppose that the algorithm is given $\mathcal{G},\bm{X},Y$ - we show that at each step of the algorithm, returning $\mathscr{O}^X$ would satisfy the theorem.

    In the base case $\mathscr{O}^X$ is empty, making  $\bm{O}^{X'}=\emptyset$, so $\bm{X}'=\bm{X}\cap \bm{O}^{X'} = \emptyset$. There is therefore a valid sequential $\pi$-backdoor of size 0.

    Next, suppose that $\mathscr{O}^X$ can be used to construct a valid sequential $\pi$-backdoor. Suppose we are now checking a node $V_i\in \bm{V}$ for inclusion in $\mathscr{O}^X$, following \Cref{alg:seq_pi_backdoor}.
    
    If the check fails, no node is added, and the theorem remains true. We therefore focus on the situations where an element is added to $\mathscr{O}^X$. 

    Suppose $ch(V_i)\subseteq keys(\mathscr{O}^X)$, and the algorithm chooses the earliest element of $\mathscr{O}^X[ch(V_i)]$ in temporal order, or the element is a boundary action of the current $\bm{V}^X$. For $V_i$ to be added to the keys of $\mathscr{O}^X$, we will show that the resulting conditioning set corresponds to a valid sequential $\pi$-backdoor. If the added element was in $\bm{X}$, but is not a boundary action, then we know it satisfies condition (2), since by the given construction, all directed paths from $V_i$ to $Y$ pass through elements of $\bm{X}$, which in turn don't have any descendants of $V_i$ in their conditioning sets. Furthermore, all previously added elements of $keys(\mathscr{O}^X)\cap \bm{X}$ that have all children in $keys(\mathscr{O}^X)$ satisfy condition (2), since no elements were removed from $keys(\mathscr{O}^X)$. We therefore only need to prove that the boundary actions satisfy (1). 
    
    We will prove this by contradiction. Suppose that $V_i$ is added to $\mathscr{O}^X$, but after adding $V_i$, there is a boundary action $X_j$ which had $(X_j\indep Y|\bm{Z}_j)$ before $V_i$ was added, but has $(X_j\not\indep Y|\bm{Z}_j)$ after it was added. Using \Cref{lemma:markovboundary}, we know that the only difference in $\bm{Z}_j$ before and after $V_i$ is added to $keys(\mathscr{O}^X)$ is that $V_i$ is removed from the conditioning set, and elements of its c-component and its parents that are not in $keys(\mathscr{O}^X)$  added. Because $X_j$ and $Y$ are no longer independent, there exists a path from $X_j$ to $Y$ in $\mathcal{G}'_j$ with colliders at elements of $\bm{Z}_j$. Since the entire conditioning set remains identical as before, and was a valid markov boundary, adding the elements of $V_i$'s c-component cannot open any paths to $Y$. However, the removal of $V_i$ from the conditioning set can open paths. We therefore know that the path from $X_j$ to $Y$ must pass through $V_i$. Suppose $P$ is this path. There are two possibilities for this path.
    
    \begin{enumerate}
    \item The path comes to $V_i$, and continues into the descendants to $V_i$ ($V_i\rightarrow ...$). All paths into descendants pass to either elements of $\bm{X}$ that come after $X_j$, in which case they are not ancestors of $Y$ in $\mathcal{G}'_j$, and $\bm{Z}_j$ does not condition on them, meaning that the path can't get to $Y$. On the other hand, if the path passes to elements of $\bm{X}\cap \before(X_j)$, it has a collider at that element (call it $X_l$), and then continues back up. However, if the path continues back passing $V_i$ again, we know that it must be blocked, since in the original conditioning set, we can modify the path to simply use $V_i$ as a collider, showing a contradicton. On the other hand, if the path does not pass back up to $V_i$'s ancestors, either $(X_l\not\indep Y|\bm{Z}_l)$, in which case we can repeat this proof using $X_l$ instead of $X_j$ as the starting node (since $\bm{Z}_l\subset \bm{Z}_j$), or the path uses an element $X_o\in \after(X_l)$ but $X_o\in \before(X_j)$ as a collider. In that case, the same argument can be repeated: either $(X_o\not\indep Y|\bm{Z}_o)$, in which the proof can be restarted with $X_o$, or the path continues to another such element. Since there are finite elements of $\bm{X}$, at some point we have $(X_o\not\indep Y|\bm{Z}_o)$, and can restart the proof from there.

    \item The path comes to $V_i$ from the descendants ($\leftarrow V_i \leftarrow$) or $V_i$ is the starting node. The path must therefore either start at a descendant to $V_i$ ($X_l$) or have a collider at $X_l$. In both cases, since $V_i$ passed the conditioning check that includes all such possible descendants, the set $\bm{Z}_l$ contains all the elements of the c-component and their parents that are not in $keys(\mathscr{O}^X)$. We can therefore repeat the argument made in possibility 1 for the continuation of the path, showing that there must exist another element $X_o$ where $(X_o\not\indep Y|\bm{Z}_o)$ along this path, from which the proof can be restarted.
    \end{enumerate}
    
    Since both cases recusively shorten $P$ on each restart of the proof, there will be an $X_o$ at which one of the requirements will be violated, showing a contradiction.
\end{proof}

\alghasmfactor*
\begin{proof}
    \Cref{lemma:fullvx} shows that $\bm{X}\subseteq\bm{O}^{X}$, if a $\pi$-backdoor exists, and \Cref{thm:constructmfactor} shows that we can construct a valid $\pi$-backdoor whenever $\bm{X}\subseteq\bm{O}^{X}$, which shows that the algorithm returns an answer if and only if a $\pi$-backdoor exists.
\end{proof}
\begin{lemma}
    \label{lemma:subsetoutput}
    $\bm{O}^{X}:=\textsc{FindOx}(\mathcal{G},\bm{X},Y)$, and let $\bm{O}^{X'}:=\textsc{FindOx}(\mathcal{G},\bm{X}',Y)$, with $\bm{X}'\subseteq \bm{X}$. Then $\bm{O}^{X'}\subseteq \bm{O}^{X}$.
\end{lemma}

\begin{proof}
    We first observe that keys can only be added to $\mathscr{O}^X$ in \Cref{alg:seq_pi_backdoor}. Furthermore, we observe that the conditioning checks can only be helped by adding values of $\bm{X}$ to consider in the algorithm (i.e. adding an element to $\mathscr{O}^X$ cannot cause a conditioning check to fail that would otherwise succeed, but it can cause a conditioning check to succeed where it would have failed). Therefore, all of the conditioning checks that succeeded when using $\bm{X}'$ will also succeed when using $\bm{X}$, and so $keys(\mathscr{O}^{X'})\subseteq keys(\mathscr{O}^{X})$.
\end{proof}

\biggestmfactor*

\begin{proof}
    Suppose not, that is, suppose that a sequential $\pi$-backdoor exists for $\bm{X}"$, but $\bm{X}"\not\subseteq \bm{V}^X$. However, using \Cref{lemma:subsetoutput}, it also means that $\bm{V}^{X"}:=\textsc{FindOx}(\mathcal{G},\bm{X}",Y)$ does not contain $\bm{X}"$, and so using \Cref{thm:alghasmfactor}, no sequential $\pi$-backdoor exists for $\bm{X}"$, a contradiction.
\end{proof}

==> a_experiments.tex <==

This section describes implementation details of each experiment.

\subsection{Synthetic Binary Simulations}
\label{sec:binary_experiments}
This experiment first generates a randomly sampled model consistent with the causal graphs in \Cref{tbl:simulations}. All variables are binary. This means that each variable $X$ contains 2 possible actions. $Y$ is also binary, such that $\E[Y]$ is sufficient for characterizing the imitation results.

For each variable in the causal graph, the model was generated by sampling each element of the conditional probability table (CPT) uniformly at random. For example, $X_2$ in \Cref{tbl:simulations} \#1 would have its CPT generated as follows for every combination of values $x_1,u_2$ of its parents:

\[
\begin{aligned}
P(X_2=1 |X_1=x_1,U_2=u_2) &= Uniform(0,1)
\end{aligned}
\]

Y was also generated in the same way:
\[
\begin{aligned}
P(Y=1|Pa(Y)) &= Uniform(0,1)\\
P(Y=0|Pa(Y)) &= 1 - P(Y=1|Pa(Y))\\
\end{aligned}
\]

This type of modeling ensures that the resulting bias is an average of randomly chosen models, proving that distributions where the bias is non-negligible consistent with the given graphs are common.

With the models produced as above, for each action, we sampled 10,000 runs, creating a dataset over the observed variables (including expert actions). We subsequently found the empirical CPT for each action $X_i$ to reproduce $P(X_i|Context)$ from the observational data. Context is chosen according to the given policy (Seq $\pi$-Backdoor, $\pi$-Backdoor, Observed Parents, All Observed).

Finally, the trained policies were plugged back into the model, giving their performance in the actual system for a total of 10000 runs. The absolute value of the difference between the expectation of $Y$ from expert and the imitator is recorded.

This procedure, including sampling of new models consistent with the graph, is performed 1000 times for each graph, and the resulting average performance is recorded in \Cref{tbl:simulations}.

\subsection{Adversarial Graph with Continuous Data}
\label{sec:highd}

\begin{figure}
        \centering
        \begin{tikzpicture}
            \node[vertex,dashed,red,thick] (y) at (-4,-2) {$Y$};

            \node[vertex] (v4) at (-1,0) {$R_4$};
            \node[vertex,blue,thick] (x3) at (-2,0) {$X_3$};
            \node[vertex] (v3) at (-3,0) {$R_3$};
            \node[vertex,blue,thick] (x2) at (-4,0) {$X_2$};
            \node[vertex] (v2) at (-5,0) {$R_2$};
            \node[vertex,blue,thick] (x1) at (-6,0) {$X_1$};
            \node[vertex] (v1) at (-7,0) {$R_1$};
            
            \node[vertex,dashed] (h) at (-4,1.2) {$H$};
            \node[vertex] (q) at (-7,1) {$A$};
            \node[vertex,dashed] (c) at (-8,0) {$C$};
            
            \path (v1) edge (x1);
            \path (x1) edge (v2);
            \path (v2) edge (x2);
            \path (x2) edge (v3);
            \path (v3) edge (x3);
            \path (x3) edge (v4);
            
            \path (h) edge (x1);
            \path (h) edge (x2);
            \path (h) edge (x3);
            
            \path (h) edge (q);
            \path (c) edge (q);
            \path (c) edge[bend right=20] (y);
            
            \path (v4) edge[bend left=20] (y);
            \path (v1) edge[bend right=15] (y);
            \path (v2) edge (y);
            \path (v3) edge (y);
            
            
            \path (v1) edge[bend right=40] (v2);
            \path (v2) edge[bend right=40] (v3);
            \path (v3) edge[bend right=40] (v4);
            %\path (v1) edge[bend right=30] (y);
            
            \path (c) edge (v1);
        \end{tikzpicture}

    \caption{\label{fig:highdgraph}Causal graph for the continuous data experiment given in \Cref{sec:highd}.}
\end{figure}


The causal graph in \Cref{fig:highdgraph} was generated to demonstrate a larger problem that uses continuous observed variables rather than the small binary graphs demonstrated in \Cref{sec:binary_experiments}.

The implemented structure intuitively represents a simplified radar-based cruise control system's observations of a driver's behavior. At the time of each action $X_i$, the radar ($R_i$) detects the distance to the car in front, as well as the change in distance over time. The driver is increasing/decreasing  ($X_i$) the speed based on both the distance to the car in front, and their own mental state ($H$, for ``in a hurry''), which is unobserved by the driving system. The driver's action results in a new distance/relative velocity between cars ($R_{i+1}$).

The driving system also has access to the full vehicle state, which includes whether the air conditioning ($A$) has been turned on. The AC state is determined by the driver's internal thoughts ($H$), as well as the driving conditions ($C$), including outside temperature, which are not directly sensed by the system.

Finally, whether the driver is considered a ``safe driver" according to highway patrol is dependent on the overall conditions ($C$), and the distance between cars throughout the measuring period ($R_i$).

The goal of the system is to drive in such a way that the anti-robot highway patrol will not notice any erratic behavior.

In this model, we once again compare the 4 approaches.
\begin{enumerate}
\item \textbf{All Observed}: We assume that $A$ is observed before all actions. This gives us the following policy:
\[
\begin{aligned}
\pi(X_1|R_1,A)&=P(X_1|R_1,A)\\
\pi(X_2|R_1,X_1,R_2,A)&=P(X_2|R_1,X_1,R_2,A)\\
\pi(X_3|R_1,X_1,R_2,X_2,R_3,A)&=P(X_3|R_1,X_1,R_2,X_2,R_3,A)\\
\end{aligned}
\]
\item  \textbf{Observed Parents}: In this approach, we only condition each policy on the subset of the action's parents that are observed. Namely:
\[
\begin{aligned}
\pi(X_1|R_1,A)&=P(X_1|R_1)\\
\pi(X_2|R_1,X_1,R_2,A)&=P(X_2|R_2)\\
\pi(X_3|R_1,X_1,R_2,X_2,R_3,A)&=P(X_3|R_3)\\
\end{aligned}
\]
\item \textbf{$\pi$-Backdoor}: The $\pi$-backdoor cannot be applied in this situation, since $X_1$ would need to be imitable by itself, whereas here there is a path to $Y$ through $H$ that cannot be taken into account at $X_1$.
\item \textbf{Sequential $\pi$-Backdoor}: The sequential $\pi$-backdoor returns the following policy:
\[
\begin{aligned}
\pi(X_1|R_1,A)&=P(X_1|R_1)\\
\pi(X_2|R_1,X_1,R_2,A)&=P(X_2|R_1,X_1,R_2)\\
\pi(X_3|R_1,X_1,R_2,X_2,R_3,A)&=P(X_3|R_1,X_1,R_2,X_2,R_3)\\
\end{aligned}
\]
\end{enumerate}

The only difference between policies here is the data that is taken into account for imitation purposes. In particular, the sequential $\pi$-backdoor explicitly ignores the state of the air conditioning, which is available to it, and would alter the outcome (see the ``All Observed'' policy).

\subsubsection{Generating an Adversarial Environment}
\label{sec:adversarial_structure}
The cruise control system has no knowledge of ``correct'' behavior, and does not understand humans, wfich includes both the driver and highway patrol. Whatever policy is generated by the algorithm must therefore take into account any possible behaviors that are consistent with the causal graph.

To demonstrate the issues stemming from an incorrectly chosen covariate set, we are free to construct an adversarial model. To do this, we followed a procedure similar to \cite{zhangCausalImitationLearning2020}, maximizing error from na\"ive behavioral cloning. We first construct a binary model consistent with the above causal graph, then overlay continuous data over the $R_i$. The imitator will only have access to the continuous data, and will remain ignorant to the underlying data-generating mechanics, except for the causal graph. 
In particular, we will focus on two sub-structures in the model.

\begin{enumerate}
    \item The first sub-structure, shown in \Cref{fig:adversarial_backdoor}, can have the following binary representation:
    \[
    \begin{aligned}
        R_1 &\sim Bern(0.5)\\
        H &\sim Bern(0.5)\\
        X_1 &= R_1\oplus H\\
        R_2 &= X_1\\
        X_2 &= R_2\oplus H\\
        R_3 &= X_2\\
        Y &= R_1== R_3
    \end{aligned}
    \]
    Given this structure, using only $R_2$ as $X_2$'s parent when imitating will give $P(X_2|R_2)=P(X_2)$, but the correct policy would be $X_2=R_1$ - meaning that the imitator can only guess correctly half the time.
    \item The second sub-structure, from \Cref{fig:adversarial_collider}, has the following binary representation:
    \[
    \begin{aligned}
        H &\sim Bern(0.62)\\
        C &\sim Bern(0.62)\\
        A &= C\wedge H\\
        X_3 &= H\\
        R_4 &= X_3\\
        Y &= R_4\oplus C\\
    \end{aligned}
    \]
    With this structure, not including $A$ in $X_3$'s policy gives an average performance $E[Y]=0.47$, but including it gives a maximum of $E[Y|do(\pi)]=0.18$.
\end{enumerate}

\begin{figure}
\centering
\null
    \begin{subfigure}{0.48\linewidth}
        \centering
        \begin{minipage}{0.99\textwidth}
\begin{adjustbox}{max totalsize={.99\textwidth}{10cm},center}
\centering
        \begin{tikzpicture}
            \node[vertex,dashed,red,thick] (y) at (-4,-2) {$Y$};

            \node[vertex,opacity=0.1] (v4) at (-1,0) {$R_4$};
            \node[vertex,blue,thick,opacity=0.1] (x3) at (-2,0) {$X_3$};
            \node[vertex] (v3) at (-3,0) {$R_3$};
            \node[vertex,blue,thick] (x2) at (-4,0) {$X_2$};
            \node[vertex] (v2) at (-5,0) {$R_2$};
            \node[vertex,blue,thick] (x1) at (-6,0) {$X_1$};
            \node[vertex] (v1) at (-7,0) {$R_1$};
            
            \node[vertex,dashed] (h) at (-4,1.2) {$H$};
            \node[vertex,opacity=0.1] (q) at (-7,1) {$A$};
            \node[vertex,dashed,opacity=0.1] (c) at (-8,0) {$C$};
            
            \path (v1) edge (x1);
            \path (x1) edge (v2);
            \path (v2) edge (x2);
            \path (x2) edge (v3);
            \path[opacity=0.1] (v3) edge (x3);
            \path[opacity=0.1] (x3) edge (v4);
            
            \path (h) edge (x1);
            \path (h) edge (x2);
            \path[opacity=0.1] (h) edge (x3);
            
            \path[opacity=0.1] (h) edge (q);
            \path[opacity=0.1] (c) edge (q);
            \path[opacity=0.1] (c) edge[bend right=20] (y);
            
            \path[opacity=0.1] (v4) edge[bend left=20] (y);
            \path (v1) edge[bend right=15] (y);
            \path[opacity=0.1] (v2) edge (y);
            \path (v3) edge (y);
            
            
            \path[opacity=0.1] (v1) edge[bend right=40] (v2);
            \path[opacity=0.1] (v2) edge[bend right=40] (v3);
            \path[opacity=0.1] (v3) edge[bend right=40] (v4);
            %\path (v1) edge[bend right=30] (y);
            
            \path[opacity=0.1] (c) edge (v1);
        \end{tikzpicture}
        \end{adjustbox}
        \end{minipage}
        \caption{\label{fig:adversarial_backdoor}}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\linewidth}
        \centering
        \begin{minipage}{0.99\textwidth}
\begin{adjustbox}{max totalsize={.99\textwidth}{10cm},center}
\centering
        \begin{tikzpicture}
            \node[vertex,dashed,red,thick] (y) at (-4,-2) {$Y$};

            \node[vertex] (v4) at (-1,0) {$R_4$};
            \node[vertex,blue,thick] (x3) at (-2,0) {$X_3$};
            \node[vertex,opacity=0.1] (v3) at (-3,0) {$R_3$};
            \node[vertex,blue,thick,opacity=0.1] (x2) at (-4,0) {$X_2$};
            \node[vertex,opacity=0.1] (v2) at (-5,0) {$R_2$};
            \node[vertex,blue,thick,opacity=0.1] (x1) at (-6,0) {$X_1$};
            \node[vertex,opacity=0.1] (v1) at (-7,0) {$R_1$};
            
            \node[vertex,dashed] (h) at (-4,1.2) {$H$};
            \node[vertex] (q) at (-7,1) {$A$};
            \node[vertex,dashed] (c) at (-8,0) {$C$};
            
            \path[opacity=0.1] (v1) edge (x1);
            \path[opacity=0.1] (x1) edge (v2);
            \path[opacity=0.1] (v2) edge (x2);
            \path[opacity=0.1] (x2) edge (v3);
            \path[opacity=0.1] (v3) edge (x3);
            \path (x3) edge (v4);
            
            \path[opacity=0.1] (h) edge (x1);
            \path[opacity=0.1] (h) edge (x2);
            \path (h) edge (x3);
            
            \path (h) edge (q);
            \path (c) edge (q);
            \path (c) edge[bend right=20] (y);
            
            \path (v4) edge[bend left=20] (y);
            \path[opacity=0.1] (v1) edge[bend right=15] (y);
            \path[opacity=0.1] (v2) edge (y);
            \path[opacity=0.1] (v3) edge (y);
            
            
            \path[opacity=0.1] (v1) edge[bend right=40] (v2);
            \path[opacity=0.1] (v2) edge[bend right=40] (v3);
            \path[opacity=0.1] (v3) edge[bend right=40] (v4);
            %\path (v1) edge[bend right=30] (y);
            
            \path[opacity=0.1] (c) edge (v1);
        \end{tikzpicture}
        \end{adjustbox}
        \end{minipage}
        \caption{\label{fig:adversarial_collider}}
    \end{subfigure}
    \null
    \caption{ The two sub-structures that are adversarially optimized in the binary model to generate the full causal graph.}
\end{figure}


Combining these two substructures gives us the following binary version of the full graph:
\[
\begin{aligned}
C &\sim (Bern(0.5),Bern(0.62))\\
H &\sim (Bern(0.5),Bern(0.62))\\
A &= C[1]\wedge H[1]\\
R_1 &= C[0]\\
X_1 &= R_1\oplus H[0]\\
        R_2 &= X_1\\
        X_2 &= R_2\oplus H[0]\\
        R_3 &= X_2\\
        X_3 &= H[1]\\
        R_4 &= X_3\\
        Y &= (R_1== R_3)\wedge(R_4\oplus C[1])
\end{aligned}
\]

Since the resulting samples of the above model would be binary, we generate an overlay of continuous data which has identical underlying mechanics.

\subsubsection{Applying Continuous Data to a Binary Structure}

While we could sample from arbitrary continuous distributions, we choose to use data from the HighD dataset \cite{highDdataset}, which includes vehicle trajectories gathered from drones flying over a section of highway. This dataset does not include a causal graph, and hypothesizing a graph from the data is beyond the scope of our contribution. Instead, since this data does not conform to the distribution implied by the adversarial binary structure generated in \cref{sec:adversarial_structure}, we alter the data to match the adversarial structure before performing imitation. This gives us a non-trivial continuous distribution conforming to the causal graph. We are effectively creating a new dataset using the randomness/distribution present in the HighD dataset's trajectories, for which we know the ground-truth causal diagram and model.

The procedure used to generate a trajectory conforming to a sequence of actions determined by the causal model from a trajectory in the HighD dataset is:

\begin{enumerate}
    \item Sample each real trajectory at 4 points (one for each $R_i$), giving a tuple for the distance/change of distance between cars $((D_1,\Delta D_1)(D_2,\Delta D_2),(D_3,\Delta D_3),(D_4,\Delta D_4))$.
    \item Set each new trajectory to be $D'_i = D_1 + \sum_{j=2}^i |\Delta D_j|\times (-1)^{1-X_j}$ based on the actions, with $\Delta D_i = |\Delta D_i|\times (-1)^{1-X_{i-1}}$.
\end{enumerate}

This gives continuous trajectories conforming to the adversarial causal model.

By using $Y=((\Delta D_1 >0)==(\Delta D_3 >0)) & ((\delta D_4 >0)^C[1])$, we get a simulator for trajectories, and can use the above conversion to evaluate imitator decisions.

\subsubsection{Imitators}

A 2 hidden layer neural network with (50,20) neurons with ReLU activation, and Adam optimizer (lr=$5e-5$) was trained for each $X_i$ and context pair. At each $X_i$, the network inputs were the context variables specific to the method being tested, and output being a prediction of probability of $X_i$ (sigmoid activation with BCE loss).

The outputs ($X_1,X_2,X_3$) were binarized by sampling from a bernoulli distribution using the outputs of the network as probabilities.

\subsubsection{Results}

The testing dataset was converted using the same method as described above, using the outputs $X_1,X_2,X_3$ from the learned policies instead of the ground-truth causal graph as inputs to the synthetic trajectory generation. This gave an expected performance average for each policy type, shown in \Cref{fig:highd_resuls}.


==> a_necessity.tex <==


\begin{definition}
    \label{def:advpath}
    A $\mathscr{O}^X$-adversarial directed path is a directed path from a node $V_1$ to $Y$ in the ancestral graph of $Y$,
    such that given $\mathscr{O}^X$ from $\textsc{FindOx}(\mathcal{G},\bm{X},Y)$, is constructed iteratively starting from $V_i$ as follows:
    \begin{itemize}
        \item If $ch(V_i)\subseteq keys(\mathscr{O}^X)$, choose the one that maps to the earliest element of $\bm{X}$ in $\mathscr{O}^X$ ($V_{i+1} \in \{V_j| V_j\in ch(V_i), \mathscr{O}^X[ch(V_i)] \subseteq \after(\mathscr{O}^X[V_{j}]) \}$)
        \item If $\bm{V}_c := ch(V_i)\setminus keys(\mathscr{O}^X)$ is non-empty, choose any $V_{i+1}\in \bm{V}_c$ as next element in path.
        \item If the resulting path intersects with another, the path continues with the other to $Y$.
    \end{itemize}
\end{definition}


\begin{definition}
    \label{def:advpathset}
    A $\mathscr{O}^X$-adversarial directed path set is a set of paths starting at a set of nodes $\bm{V}^P$ to $Y$, where each path carries a tuple of values, and two paths merging concatenates the tuples of both paths, such that $Y$ obtains a tuple containing all of the values of nodes at $\bm{V}^P$.
\end{definition}

\begin{definition}
    A $\mathscr{O}^X$-adversarial latent path is a path starting at $V_i\in \bm{V}^Y$ and ending at $V_j\in \bm{V}^Y$, of the form $V_i \leftarrow ... \rightarrow C_1 \leftarrow ... \rightarrow V_j$, with colliders $C_1,C_2,...,C_k \in \bm{C} \subseteq \bm{V}^Y$ and:
    \begin{enumerate}
        \item $\forall C_i \in \bm{C}\cup\{V_i,V_j\}, C_i \notin keys(\mathscr{O}^X)$
        \item All elements along the path except $\bm{C},V_i,V_j$ are latent
        \item $V_j$ comes after $V_i$ and all elements of $\bm{X}$ where $\{X_i \in \bm{X} | \exists C_i \in \bm{C}\cup\{V_i\}, ch(C_i) \subseteq keys(\mathscr{O}^X), X_i \in \mathscr{O}^X[C_i], X_i \in \Before(X_j) \forall X_j\in \mathscr{O}^X[C_i]\}$
        \item $|ch(V_j)\setminus keys(\mathscr{O}^X)| > 0$
    \end{enumerate}
\end{definition}

\begin{lemma}
    \label{lemma:advlatentpath_exists}
    Given $\mathscr{O}^X$, and $V_i\in \bm{X}$ or $ch(V_i) \subseteq keys(\mathscr{O}^X)$, but $V_i\notin keys(\mathscr{O}^X)$, then there exists a $\mathscr{O}^X$-adversarial latent path from $V_i$ to a node $V_j$, crossing colliders $A_1,...,A_k$.
\end{lemma}

\begin{proof}
    Given the c-component $\bm{C}$ of $V_i$ (including $V_i$), every $C_i\in \bm{C}$ which is not in $keys(\mathscr{O}^X)$, but is either in $\bm{X}$ or has all its children in $keys(\mathscr{O}^X)$ had $(V_i\indep \bm{C}\setminus (\bm{O}^X \cup\{V_i\})| (\bm{C}\setminus(\bm{O}^X \cup\{V_i\}))\cap\before(X_i))$ in $\mathcal{G}_{\bm{C}}$ evaluated in $\textsc{FindOx}(\mathcal{G},\bm{X},Y)$ on the last iteration, and failed the check, without any changes to $\mathscr{O}^X$ in the iteration. This means that each $C_i$ has an element of the c-component, $C_j \in \after(C_i)$ (otherwise it would be part of the conditioning in the check) such that there is a path in the c-component's subgraph to it crossing only colliders $A_1,...,A_k\in \bm{C}$ not in $\mathscr{O}^X$.

    Let $P$ be the path corresponding to $V_i$. Conditions 1,2 hold by definition. However, this path does not necessarily satisfy conditions 3,4. Let $A_i$ be the first element along the path from $V_i$ which violates condition 3, meaning that $V_j$ comes before $A_i$. Since $A_i$ must is either in $\bm{X}$ or has all its children in $keys(\mathscr{O}^X)$ by the requirements of condition 3's constraint, it has a path to a different end element, $V_a$, which comes after $A_i$. We can therefore concatenate $P$ with the new path, removing all loops and intersections, such that we are left with a new path $P'$ ending at $V_a$. The elements of the path before $A_i$ satisfied condition 3, so they must satisfy the condition with an end element coming even later in temporal order. We can repeat this procedure until we have a path from $V_i$ where none of the colliders come after the last element $V_j'$, meaning that condition 3 is also satisfied.

    Finally, suppose $V_j$ has all of its children in $keys(\mathscr{O}^X)$, violating condition 4. This is once again sufficient for a path to exist from $V_j$ to an element before $V_j$, which is concatenated in the same manner to $P$. We repeat the procedure for violations of 3 and 4 until all conditions are satisfed (which can be repeated up to $|\bm{C}|$ times, since each iteration uses a later end node in the c-component).

    The above procedure is sufficient for the resulting path to be a $\mathscr{O}^X$-adversarial latent path starting from $V_i$, which completes the proof.
\end{proof}

\notimitablealgorithm*

\begin{proof}
    We prove this by induction, starting with a proof that $\bm{X}\cap \Before(X_i)$ is not imitable.

    \textbf{Base Case:} Define $X_j$ to be the earliest element of $\mathscr{O}^X[ch(X_i)]$ if all children of $X_i$ are in $\mathscr{O}^X$, otherwise let it be $X_i$.

    Since $X_i$ was not in $\bm{O}^{X}$, it means that there is a $\mathscr{O}^X$-adversarial latent path from $X_i$ to element $V_j\in \after(X_j)$, crossing colliders $A_1,...,A_k$ (\Cref{lemma:advlatentpath_exists}). Between each two successive observed nodes of the latent path, there is a latent variable that is a common ancestor. That is, the path is of the form $X_i \leftarrow ... \leftarrow U_1 \rightarrow ... \rightarrow A_1 \leftarrow .... \rightarrow V_j$. The set of these latent variables can be $\{U_1,U_2,...,U_{k+1}\} = \bm{U}^{X_i}$. Set these variables to each be $U_i \sim Bern(0.5)$ (i.e. random coin flips), and have the directed paths from $\bm{U}^{X_i}$ to the observed nodes of the path to simply pass through the values. Then, let each $A_i=U_{i}\oplus U_{i+1}$, $X_i = U_1$, and $V_i = U_{k+1}$. Finally, construct a $\mathscr{O}^X$-adversarial directed path set (\Cref{def:advpathset}) from $(\bm{A}...,V_i,X_i)$ to $Y$ that passes these values to $Y$. $Y$ then accepts the set of values $(\bm{A}...,V_i,X_i)$ which conform to the condition $0=X_i\oplus V_j\oplus\bigoplus_{A_i\in\bm{A}} A_i$. Note that we do not have $Y$ as a mathematical function of its arguments, but rather as the set of tuples that are considered "correct", with $Y=1$ if the inputs to $Y$ are in the ``accepted'' set, and $Y=0$ otherwise.

    When the expert is acting, the result is is 0, since $M\oplus M=0$ for any variable $M$, making $Y=1$:
    \[
        X_i \oplus \left(\bigoplus_{A_i\in\bm{A}} A_i \right)\oplus V_j = U_1\oplus (U_1 \oplus U_2) \oplus (U_2 \oplus U_3) \oplus...\oplus (U_{k}\oplus U_{k+1}) \oplus U_{k+1} = 0
    \]
    We observe that when imitating $X_i$, the imitator does not have access to $U_1$, and all imitated elements can only use $\bm{A}$ as context (since $X_i$ is the last element of $\bm{X}\cap \Before(X_i)$ in temporal order, and $V_i\in \after(X_i)$. Since many paths for the path set can have crossed $X_i$, we can create a generalized imitator which has control over all of the inputs to $Y$ except for $V_j$. This means that the requirement is now:
    \[
        0= V_j \oplus f(A_1,...,A_k) = U_{k+1}\oplus f(U_1 \oplus U_2,...,U_{k}\oplus U_{k+1})
    \]
    $U_{k+1}$ is only present in $A_k$, but then $U_{k}$ must be isolated to extract the value of $U_{k+1}$. This proceeds recursively along the chain until $U_1$ is reached, which is not present in any other observed variable, allowing us to conclude that it is impossible to isolate $U_{k+1}$, and therefore impossible to guess correctly all the time, and so it is impossible to match the expert's performance (which is 100\%). We have therefore shown that $\bm{X}\cap \Before(X_i)$ is not imitable.


    \textbf{Inductive Step:} Define $X_{j}\in \bm{X}$. Suppose that $\bm{X}\cap \before(X_j)$ is not imitable, with a given adversarial circuit for $\bm{X}\cap \before(X_j)$ as constructed in this proof bearing witness to non-imitability. We will prove that $\bm{X}\cap \Before(X_j)$  (i.e. including $X_j$) is not imitable, and construct a corresponding circuit.

    We are adding another imitator $X_j$ to the previous path sets, which can possibly come after the previous circuit's adversarial path $V_j$ (which came after $X_{j-1}$). This means that we must modify the circuit to make sure that $X_j$ cannot use its ability to observe previous values to ``fix'' any mistakes made by $X_{j-1}$.

    If none of the paths from the previous circuit pass through $X_j$, then it cannot affect the value of $Y$, and thus $\bm{X}\cap \Before(X_j)$ is not imitable with an identical circuit as the previous inductive step. Similarly, any adversarial directed paths that enter $\bm{O}^X$ in the second node of the path and move across $X_j$ before exiting to $\bm{V}^Y$ (first node of any adversarial directed path in the circuit is never in $\bm{O}^X$) means that there is an element in $\after(X_j)$ in the $\mathscr{O}^X$-adversarial latent path that created the node starting this path set, and therefore $X_j$ cannot know at least one of the values required to ``correct'' for the value passed down this path (each adversarial latent path corresponds to a sequence of xors of bernoulli random variables - to set these values to be consistent with the full xor chain, $X_j$ would need to have access to the entire chain).

    Finally, suppose there is a set $\bm{P}$ of $\mathscr{O}^X$-adversarial directed paths which enters $\bm{O}^X$ and passes through $X_j$ before exiting to $\bm{V}^Y$, and the last node $V_b$ of each such path before entering $\bm{O}^X$ to $X_j$ is not the first node of the path. Note that the value of $\mathscr{O}^X$ stays the same in each fragment of $\bm{O}^X$ before exiting to $Y$, since otherwise it would mean that either the path moved across a boundary node directly back into $\bm{O}^X$ (disallowed by definition of adversarial path), or that the conditioning check succeeded using $V_i,V_i$, but failed when using $X_i,V_i$, where $X_i$ comes after $V_i$ - where there are less elements not conditioned. For each path $p_i\in \bm{P}$ we have two cases. In the first case, the path did not cross any other $X_i$ after entering the $\bm{O}^X$ of $X_j$, and in the second case it does.

    We start by tackling the first case. We know that $\bm{X}\cap \before(X_j)$ is not imitable, so with a certain probability, the full set of paths gives a set of values that are not in the acceptable set for $Y$. In particular, it is now possible that by modifying the values that pass through the paths across $X_j$, the imitator might set the values to their correct settings given the context of all previous values. The adversary can prevent this by recognizing that $V_b$ (the last node of $p_i$ before entering $\bm{O}^X$ to $X_j$) must have an associated $\mathscr{O}^X$-adversarial latent path from $V_b$ to element $V_j\in \after(X_j)$. Suppose that the path $p_i$ passes $n$ binary values to $Y$ across $V_b$. We combine this with an adversarial latent path, which is of the form $V_b \leftarrow ... \leftarrow U_1 \rightarrow ... \rightarrow A_1 \leftarrow .... \rightarrow V_j$. The set of these latent variables can be $\{U_1,U_2,...,U_{k+1}\} = \bm{U}^{X_i}$. Set these variables to each be $U_i \sim Bern(0.5)^{2n}$ (i.e. $2n$ random coin flips), and have the directed paths from $\bm{U}^{X_i}$ to the observed nodes of the path to simply pass through the values.
    Once again, each $A_i=U_{i}\oplus U_{i+1}$ where the xor is performed elementwise, and $V_i = U_{k+1}$. At $V_b$, however, we now perform a different operation. We take the $2n$-dimensional vector coming from $U_1$, reshape it to $(n,2)$, and have as output be $U_1[p_i]$, in other words, the binary values passing through $p_i$ are now indices that choose the binary values from $U_1$ for each element. In other words, if $p_1$ carries the tuple $(0,1)$, and $U_1 = \begin{pmatrix}a & b\\c & d\end{pmatrix}$, then $U_1[p_1] = (a,d)$. Then, the path $p_i$ replaces its value at $V_b$ with this output, carrying it to $Y$. At $Y$, each element of the set of valid values has its corresponding $p_i$ element replaced with the set of values compatible with:
    \[
        0= V_b[p_i] \oplus \left(\bigoplus_{A_i\in\bm{A}} A_i[p_i] \right)\oplus V_j[p_i]
    \]

    This is because once again:
    \[
        U_1[p_i]\oplus (U_1 \oplus U_2)[p_i] \oplus (U_2 \oplus U_3)[p_i] \oplus...\oplus (U_{k}\oplus U_{k+1})[p_i] \oplus U_{k+1}[p_i] = 0
    \]

    Once again, without being able to change the value of $p_i$ to the correct one \textit{before} it gets to $V_b$, $X_j$ only has access to the \textit{imitated} value of $p_1$, which only matches the correctly imitated elements. Without knowledge of $V_j$, $X_j$ cannot correctly account for the elements of $p_j$ which were not imitated/guessed correctly (inductive hypothesis).

    Finally, in the second case, the path crossed through another element $X_i$ after entering the $\bm{O}^X$ of $X_j$. This means that $\mathscr{O}^X$ at $V_b$ for $X_i$ was either $X_j$ or an element after it, meaning that the circuit constructed for $X_i$ still has its $V_i$ value unobserved by $X_j$, and once again cannot be imitated.

    By repeating this step for each path crossing $X_j$, and performing the procedure for each $X_j\in \bm{X}$, we can construct a full circuit for the entire graph, which is not imitable at each step in temporal order after the element $X_i$, completing the proof.
\end{proof}

\seqpibackdoornecessary*

\begin{proof}
    By \Cref{thm:alghasmfactor} and \Cref{thm:notimitablealgorithm}
\end{proof}

==> a_sufficiency.tex <==
The proof of sufficiency will make heavy use of sufficiency of the $\pi$-backdoor as shown in \cite{zhangCausalImitationLearning2020}, reproduced here using our paper's notation for convenience:

\begin{theorem}
\label{thm:pibackdoor}
\cite{zhangCausalImitationLearning2020} $Y$ is imitable w.r.t. $X$ in $\mathcal{G}$ if there is $\bm{Z}\subseteq \before(X)$ such that $(X\indep Y|\bm{Z})$ in $\mathcal{G}_{\underline{X}}$. Moreover, the imitating policy is given by $\pi(\bm{Z})=P(X|\bm{Z})$.
\end{theorem}

We will show that the sequential version can be proved with a recursive application of \Cref{thm:pibackdoor}:

\piseqbdsufficiency*

\begin{proof}
    We will proceed by induction on the $\bm{X}$ in reverse temporal order. In the base case we have $\mathcal{G}'_k$ with distribution over $Y$ identical to the distribution over $Y$ in $\mathcal{G}$ ($\mathcal{G}'_k=\mathcal{G}$ so the distribution of $Y$ when no action is taken by the imitator is identical to the original distribution).
    
    In the inductive step, we have graph $\mathcal{G}'_i$, which explicitly encodes actions of $X_{i+1},...,X_k$. We know that the distribution over $Y$ is identical in both $\mathcal{G}$ and $\mathcal{G}_{i}$.
    
    If condition (2) is satisfied for $X_i$ in $\mathcal{G}_{i}$, then $X_i$ is not an ancestor of $Y$, and therefore $P(Y|do(X_i))=P(Y)$ for any action $X_i$. We can therefore take \textit{any} action from $X_i$ without affecting the distribution of $Y$, and therefore the distribution is identical for $Y$ in $\mathcal{G}$ and $\mathcal{G}_{i-1}$ (which is the graph explicitly encoding whichever policy was chosen for $X_i$.
    
    If condition (2) is not satisfied, condition (1) must be satisfied in $\mathcal{G}_{i}$, and by \Cref{thm:pibackdoor}, the policy $\pi_{X_i}(\bm{Z}_i)=P(X_i|\bm{Z}_i)$ perfectly imitates $Y$ in $\mathcal{G}_{i}$, meaning that once the policy is explicitly encoded to construct $\mathcal{G}_{i-1}$ we have $P(Y)_{\mathcal{G}_{i-1}}=P(Y)_{\mathcal{G}_{i-1}}=P(Y)_{\mathcal{G}}$ where $P(Y)_{\mathcal{G}_j}$ is the probability of $Y$ assuming the given policy is followed for $X_{j+1},...,X_k$. We therefore have $\mathcal{G}_{i-1}$ which encodes the causal graph of the imitator acting on $X_i,...,X_k$ has an identical distribution over $Y$ if the given policies are taken, proving the inductive hypothesis.
    
    Finally, once all actions are taken according to the described policies, the distribution over $Y$ remains identical to the distribution over $Y$ in the original mode with all actions taken by expert, meaning that $Y$ is imitable with respect to $\bm{X}$ in $\mathcal{G}$.
\end{proof}




\begin{comment}
\mfactor*

\begin{lemma}
    \label{lemma:msubfactor}
    Given the temporal order over the nodes in $\mathcal{G}$ and an associated m-factor $(\bm{O}^X,\bm{X},\bm{Z},Y)$, then for all $V_i\in \bm{V}$, the sets $\bm{O}^X_i = \bm{O}^X\cap \before(V_i)$, $\bm{V}^Y_i = \bm{V}^Y\cap \before(V_i)$, $\bm{X}_i = \bm{X} \cap \before(V_i)$ and $\bm{Z}_i = \bm{Z}\cap \before(V_i)$ satisfy conditions 1-4 in \Cref{def:mfactor} for the subgraph $\mathcal{G}_i$ which is made up of nodes $\before(V_i)$.
\end{lemma}

\begin{proof}
    To begin, we notice that conditions 1 holds by definition, since the subsets simply remove all nodes that come after $V_i$.

    Since temporal order is a valid topological order of the nodes, we prove conditions 2-4 by induction on the temporal order.

    \textbf{Base Case:}
    In the base case, there are no nodes in the graph, so all sets are empty. All 4 conditions are satisfied by empty sets.

    \textbf{Induction:} Suppose that \Cref{lemma:msubfactor} holds for $i-1$. The $i$th node in temporal order, $V_i\in \bm{V}$ is added. It can be in either $\bm{O}^X$ or $\bm{V}^Y$. We handle each case separately:

    \begin{itemize}
        \item Suppose $V_i\in \bm{V}^Y$. We prove the conditions by contradiction.
              \begin{enumerate}
                  \setcounter{enumi}{1}
                  \item If this is violated, then $V_i$ must be in $De(\bm{O}^X)_{\mathcal{G}_{\underline{\bm{X}^B}}}$, since it held for $i-1$. This means that there is a directed path from an element of $\bm{O}^X$ to $V_i$ in $\mathcal{G}_{\underline{\bm{X}^B}}$. This same path exists in the full graph, so $V_i\in \bm{O}^X$, a contradiction.
                  \item Suppose not, that is suppose that $(\bm{O}^X\not \indep \bm{V}^Y|\bm{Z})$. This means that there is an unblocked path between an element of $\bm{O}^X$ and $\bm{V}^Y$ in $\mathcal{G}_{\underline{\bm{X}^B}i}$. This path also exists in the full graph $\mathcal{G}_{\underline{\bm{X}^B}}$, since no future node can block an existing open path (no existing elements will be added to $\bm{Z}$ in the future). This is a contradiction, since independence holds for the full graph.
                  \item We use the same reasoning as in (3) to show that (4) holds.
              \end{enumerate}
        \item Suppose $V_i\in \bm{O}^X$.
              \begin{enumerate}
                  \setcounter{enumi}{1}
                  \item The node was added to $\bm{O}^X$, so if it held for $i-1$, and since any descendants of $V_i$ come later in temporal order,  $\left[De(\bm{O}^X)_{\mathcal{G}_{\underline{\bm{X}^B}}}\right]_{i-1} \cup \{V_i\} =\left[De(\bm{O}^X)_{\mathcal{G}_{\underline{\bm{X}^B}}}\right]_{i} \subseteq \bm{O}^X$.
                  \item We use the same reasoning as in (3) of previous portion of this proof.
                  \item If $V_i \notin \bm{X}^B$, the independence statement at $i-1$ still holds using the reasoning from (3). If $V_i \in \bm{X}^B$, suppose $(V_i\not\indep \bm{V}^Y|\bm{Z}\cap \before(X^B_i))$ (all others hold by induction on $i-1$). There is an unblocked path from $V_i$ to $\bm{V}^Y$ which still exists in the full graph, violating condition (4) for the full m-factor, a contradiction.
              \end{enumerate}
    \end{itemize}

    The conditions therefore hold for all $i$ by induction.

\end{proof}

\begin{lemma}
    \label{lemma:differentc}
    Given an m-factor $(\bm{O}^X,\bm{X},\bm{Z},Y)$ for $\mathcal{G}$, $V_i\in \bm{V}^Y\setminus \bm{Z}$ does not have any element of $\bm{O}^X$ in its c-component.
\end{lemma}

\begin{proof}
    Suppose not. That is, suppose $\exists V_x \in \bm{O}^X$ in the same c-component as $V_i$. By \Cref{def:ccomponent}, there is a path with observed colliders between $V_i$ and $V_x$.
    Take the path starting from $V_x$ to the first collider. If the element is in $\bm{O}^X$, we can shorten the path by taking this new element as the start point.
    Otherwise, the element is in $\bm{V}^Y$. Since the two are d-connected, this element must be in $Z$, otherwise condition 3 of m-factor is violated.
    Since the element is in $Z$, the path can continue to the next collider, and $V_x$ is dependent on the next element, and the argument can repeat for the remainder of the chain, leaving the endpoint $V_i$ as either part of $Z$, or dependent on $V_x$, which is a contradiction.
\end{proof}


\mfactorimitable*

\begin{proof}
    We will perform a proof by induction over the joint $P(\bm{V}^Y\cup \bm{X}^B)$, going in temporal order over $\mathcal{G}$. We will exploit \Cref{lemma:msubfactor} to claim that the subgraph at each point in temporal order satisfies claims 1-4 of \Cref{def:mfactor}.

    \textit{Inductive Hypothesis:} Given the variables until $V_i$ in temporal order, $P(\bm{V}^Y_i\cup \bm{X}^B_i)=\hat P(\bm{V}^Y_i\cup \bm{X}^B_i)$, in other words, the expert and imitator have the same distribution over $\bm{V}^Y_i$ and $\bm{X}^B_i$.

    \textit{Base Case:} When there are no nodes in the graph, $P(\emptyset)=\hat P(\emptyset)$.

    \textit{Induction:} Suppose that the inductive hypothesis holds for $i-1$. We now have 3 possible cases for the added variable $V_i$:
    \begin{itemize}
        \item $V_i \in \bm{O}^X$ but $V_i \notin \bm{X}^B$: In this case, $\bm{V}^Y_i= \bm{V}^Y_{i-1}$ and $\bm{X}^B_i=\bm{X}^B_{i-1}$, so the joint is unchanged, as no variables are added to it, so the IH holds for $i$.
        \item $V_i \in \bm{O}^X$ and $V_i \in \bm{X}^B$: In this case, $V_i$ is added to the joint. We can perform the following:
              \begin{align*}
                  P(\bm{V}^Y_i\cup \bm{X}^B_i) & = P(\bm{V}^Y_{i-1}\cup \bm{X}^B_{i-1})P(V_i|\bm{V}^Y_{i-1}\cup \bm{X}^B_{i-1})              &  & \text{Using $\bm{V}^Y_i=\bm{V}^Y_{i-1}$ and $\bm{X}^B_{i}=\bm{X}^B_{i-1}\cup\{V_i\}$} \\
                                               & =\hat P(\bm{V}^Y_{i-1}\cup \bm{X}^B_{i-1})P(V_i|\bm{V}^Y_{i-1}\cup \bm{X}^B_{i-1})          &  & \text{Inductive Hypothesis}                                                           \\
                                               & = \hat P(\bm{V}^Y_{i-1}\cup \bm{X}^B_{i-1})P(V_i|\bm{Z}_{i-1}\cup \bm{X}^B_{i-1})           &  & \text{Condition 4 and \Cref{lemma:msubfactor}}                                        \\
                                               & =\hat P(\bm{V}^Y_{i-1}\cup \bm{X}^B_{i-1})P(V_i|(\bm{X}^B\cup\bm{Z})\cap \before(V_i))      &  & \text{Rewrite in terms of before}                                                     \\
                                               & =\hat P(\bm{V}^Y_{i-1}\cup \bm{X}^B_{i-1})\hat P(V_i|(\bm{X}^B\cup\bm{Z})\cap \before(V_i)) &  & \text{This is policy used for $V_i$}                                                  \\
                                               & = \hat P(\bm{V}^Y_i\cup \bm{X}^B_i)                                                         &  & \text{Put back together to joint}
              \end{align*}
        \item $V_i \in \bm{V}^Y$ and $V_i \notin \bm{Z}$. In this case, $V_i$ is not in the same c-component $\bm{C}_i$ as any node in $\bm{O}^X$ (\Cref{lemma:differentc}). We can therefore perform a decomposition similar to \cite{tianGeneralIdentificationCondition2002a}, by splitting the joint into c-components, with all $\bm{O}^X\setminus \bm{X}^B$ considered latent. We will call this set of c-components $\bm{S}$. Consider the quantity $P(\bm{C}_i|pa(\bm{C_i}\setminus{C_i}))$. Since by the inductive hypothesis, the joint of $pa(\bm{C}_i)\setminus{C_i}$ is identical in both expert and imitator distributions. Next, we recognize that all mechanisms within the c-component conditioned on its parents are identical for both imitator and expert, meaning that their conditional joint will likewise be identical, so $P(\bm{C}_i|pa(\bm{C_i}\setminus{C_i}))=\hat P(\bm{C}_i|pa(\bm{C_i}\setminus{C_i}))$. This means that we can do the following:
              \begin{align*}
                  P(\bm{V}^Y_i\cup \bm{X}^B_i) & = \prod_{\bm{C}\in \bm{S}}P(\bm{C}|pa(\bm{C}\setminus{\bm{C}}))                                                                             &  & \text{C-component decomposition}  \\
                                               & = P(\bm{C}_i|Pa(\bm{C_i}\setminus{\bm{C}_i}))  \prod_{\bm{C}\in \bm{S}\setminus\{\bm{C_i}\}}\hat P(\bm{C}|Pa(\bm{C}\setminus{\bm{C}}))      &  & \text{Inductive Hypothesis}       \\
                                               & = \hat P(\bm{C}_i|Pa(\bm{C_i}\setminus{\bm{C}_i}))  \prod_{\bm{C}\in \bm{S}\setminus\{\bm{C_i}\}}\hat P(\bm{C}|Pa(\bm{C}\setminus{\bm{C}})) &  & \text{See reasoning above}        \\
                                               & =\hat P(\bm{V}^Y_i\cup \bm{X}^B_i)                                                                                                          &  & \text{But back together to joint}
              \end{align*}
        \item $V_i \in \bm{V}^Y$ and $V_i \in \bm{Z}$. In this case we can use the same reasoning as in the proof for $V_i \in \bm{V}^Y$ and $V_i \notin \bm{Z}$, but with additional requirements with regards to the c-component. In particular, there can now be an element  $V_x \in \bm{O}^X$ in the c-component of $V_i$ in the graph up to $i$ in temporal order. Since we concern ourselves with the graph with $\bm{O}^X\setminus \bm{X}^B$ latent, this means that observed descendants of $V_x$ can also be part of the c-component. In particular, by condition 2, these observed elements will all be in $\bm{X}^B$. However, by condition 4, these elements must come after $V_i$ (otherwise $\bm{Z}\cap \before(X^B_i)$ doesn't include $V_i$, and thus a path to an unblocked element of $\bm{V}^Y$ can be constructed). We can therefore conclude that any such element $V_x$ does not have any observed descendants in $\mathcal{G}_i$. Without any loss of generality, we can replace $\mathcal{G}_i$ with the ancestral graph of nodes $\bm{V}^Y_i\cup \bm{X}^B_i$, in which all elements $V_x$ are removed, since they aren't ancestors of observed variables (in $\mathcal{G}_i$). This means that $V_i$ once again has no elements of $\bm{O}^X$ in its c-component, so we can perform the same c-component decomposition as in the portion of the proof above giving $P(\bm{V}^Y_i\cup \bm{X}^B_i)=\hat P(\bm{V}^Y_i\cup \bm{X}^B_i)$.
    \end{itemize}

    Finally, the full joint over the variables is identical for both expert and imitator, meaning that:

    $$
        P(Y) = \sum_{\bm{V}^Y\cup \bm{X}^B \setminus \{Y\}} P(\bm{V}^Y\cup \bm{X}^B) = \sum_{\bm{V}^Y\cup \bm{X}^B \setminus \{Y\}} \hat P(\bm{V}^Y\cup \bm{X}^B) = \hat P(Y)
    $$
\end{proof}


\end{comment}
